Text2Net: Transforming Plain-text To A Dynamic Interactive Network Simulation Environment

This paper introduces Text2Net, an innovative text-based network simulation engine that leverages natural language processing (NLP) and large language models (LLMs) to transform plain-text descriptions of network topologies into dynamic, interactive simulations. Text2Net simplifies the process of configuring network simulations, eliminating the need for users to master vendor-specific syntaxes or navigate complex graphical interfaces. Through qualitative and quantitative evaluations, we demonstrate Text2Net's ability to significantly reduce the time and effort required to deploy network scenarios compared to traditional simulators like EVE-NG. By automating repetitive tasks and enabling intuitive interaction, Text2Net enhances accessibility for students, educators, and professionals. The system facilitates hands-on learning experiences for students that bridge the gap between theoretical knowledge and practical application. The results showcase its scalability across various network complexities, marking a significant step toward revolutionizing network education and professional use cases, such as proof-of-concept testing.

==> abstract.tex <==
In this work, we introduce Text2Net, a text-based computer network simulation engine, that introduces a transformative approach to computer network education. Text2Net leverages state-of-the-art large language models (LLMs) and artificial intelligence (AI) text generation tools to interpret and transform plain-text descriptions of network topologies, configurations and functionalities, into dynamic and interactive simulations. This tool utilizes natural language processing (NLP) and large language models, specifically OpenAI's ChatGPT-4T, to facilitate an intuitive interface that allows users (e.g. students, educators, and trainer/trainee engineers) to configure and interact with network simulations without the need for learning multiple simulation tools thus simplifying hands-on learning of networking. Text2Net addresses significant educational barriers by automating complex setup processes and making network learning faster, more accessible and engaging. This paper explores Text2Net's development, focusing on its innovative use of AI, the system's architecture, and its impact on network education. We provide a comprehensive evaluation of the system's usability, performance, and educational value through qualitative analyses to demonstrate its effectiveness. Text2Net is a stepping stone to potentially revolutionize computer network education.
  
